Diving into the shallows: a computational perspective on large-scale shallow learning

In this paper we first identify a basic limitation in gradient descent-based optimization methods when used in conjunctions with smooth kernels. An analysis based on the spectral properties of the kernel demonstrates that only a vanishingly small portion of the function space is reachable after a polynomial number of gradient descent iterations. This lack of approximating power drastically limits gradient descent for a fixed computational budget leading to serious over-regularization/underfitting. The issue is purely algorithmic, persisting even in the limit of infinite data. To address this shortcoming in practice, we introduce EigenPro iteration, based on a preconditioning scheme using a small number of approximately computed eigenvectors. It can also be viewed as learning a new kernel optimized for gradient descent. It turns out that injecting this small (computationally inexpensive and SGD-compatible) amount of approximate second-order information leads to major improvements in convergence. For large data, this translates into significant performance boost over the standard kernel methods. In particular, we are able to consistently match or improve the state-of-the-art results recently reported in the literature with a small fraction of their computational budget. Finally, we feel that these results show a need for a broader computational perspective on modern large-scale learning to complement more traditional statistical and convergence analyses. In particular, many phenomena of large-scale high-dimensional inference are best understood in terms of optimization on infinite dimensional Hilbert spaces, where standard algorithms can sometimes have properties at odds with finite-dimensional intuition. A systematic analysis concentrating on the approximation power of such algorithms within a budget of computation may lead to progress both in theory and practice.

==> expr/fig_hint_m.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-5mm}
  \centering
  \includegraphics[width=0.5\textwidth]{expr/hint_m_10k_index_loss_norm_2.png}
  %{figs/mnist_y_proj_e_lb_n_4.png}
  \caption{Iterations needed for converging to label vectors along each eigendirection (estimated by Eq.~\ref{eq:gd_number_iterations_i} with $\epsilon =  10^{-4}$, $10^4$ data points from HINT-M dataset)}
  \label{fig:proj-iter}
  \vspace{-5mm}
\end{wrapfigure}

==> expr/ob_best.tex <==
{\bf Comparisons on large datasets}. \label{sec:expr-sota}
In Table~\ref{tbl:best-result} we provide a comparison to some recent state-of-the-art  results, all of them using large computational resources and sometimes complex training procedures. Except for the very recent~\cite{may2017kernel}, our  method improves performance on each dataset at a small fraction of the computational budget. 


\begin{table*}[ht]
\caption{Comparison to kernel state-of-the-art  on large datasets}
\label{tbl:best-result}
\begin{threeparttable}
\begin{adjustbox}{center}
\begin{tabular}{|c|c||c|c|c||c|c|}
\hline
Dataset & Size & Method & \begin{tabular}[c]{@{}c@{}}Computing \\ Resource\end{tabular} & \begin{tabular}[c]{@{}c@{}}Method\\ Error\end{tabular} & \begin{tabular}[c]{@{}c@{}}EigenPro\\ Error\end{tabular} & \begin{tabular}[c]{@{}c@{}}Epoch/GPU Hours\\GTX Titan GPU\end{tabular} \\ \hline
MNIST-8M & $1 \cdot 10^6$ & PCG~\cite{avron2016faster} & 42 r3.8xlarge$^{(1)}$ & $0.72\%$ & $0.70\%$ & 16 / 3.2 \\ \hline
\multirow{4}{*}{TIMIT} & \multirow{4}{*}{$2 \cdot 10^6$} & Ensemble~\cite{huang2014kernel} & IBM BlueGene/Q$^{(2)}$ & $33.5\%$ & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}$32.6\%^\dagger$\\ $(33.39\%)$\end{tabular}} & \multirow{4}{*}{10 / 3.9} \\ \cline{3-5}
 &  & BCD~\cite{tu2016large} & 128 r3.2xlarge$^{(3)}$ & $33.5\%$ &  &  \\ \cline{3-5}
 &  & Kernel~\cite{may2017kernel} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Cluster of \\ g2.2xlarge$^{(4)}$\end{tabular}} & $30.9\%$ &  &  \\ \cline{3-3} \cline{5-5}
 &  & DNN~\cite{may2017kernel} &  & $32.4\%$ &  &  \\ \hline
SUSY & $4 \cdot 10^6$ & Hierarchical~\cite{chen2016hierarchically} & IBM POWER8 & $\approx 20\%$ & $19.8\%$ & 0.6 / 0.1 \\ \hline
\end{tabular}

\end{adjustbox}
\begin{tablenotes}
\small
\item $(1)$ Each r3.8xlarge instance has 32 vCPUs and 244 GiB memory.
$(2)$ Each BlueGene/Q Nodecard contains 32 nodes $\times$ 16 cores per node.
$(3)$ Each r3.2xlarge instance has 8 vCPU and 61GiB memory.
$(4)$ Each g2.2xlarge has 1 GPU, 8 vCPU, and 15 GiB memory.
\item $\dagger$ Our TIMIT training set is generated by the standard practice in speech community~\cite{povey2011kaldi}.
It adopts 10ms frames and drops the glottal stop 'q' related labels, thus we ignore the relevant frames in core test set ($1.2\%$ of total test set).
Note that in the worst case, if we mislabel all these frames, the corresponding frame-level classification error will drop from $32.6\%$ to $33.39\%$.
\end{tablenotes}
\end{threeparttable}
\end{table*}



% One distinguishing property of RKHS kernel is its capability to accurately approximate any smooth function given enough number of centers, or in the setting of shallow learning, the number of training points.
% However, kernel methods running on large datasets rarely yield high accuracy results, especially when comparing to results from DNN. Researchers have since tried to combine preconditioning techniques with batch or online iterative methods to diminish the resource demand of kernel methods and expand its computational reach.
% Unfortunately, there are still only a few work on kernel methods by far that report high accuracy results on large dataset, e.g. results in Table~\ref{tbl:best-result}.
% What' worse, all such work tends to stack up hardwares to allow a larger computational reach.

% In contrast, our approach, frugally using a single GPU, covers even larger computational reach under a highly affordable time budget.
% The results in Table~\ref{tbl:best-result} has two implications. First, accurate large-scale shallow learning is achievable under limited resource/time budget,
% which makes it one step closer to the capability of DNN.
% Second, the concept of computational reach plays a key role in understanding and overcoming the bottlenecks of shallow learning. It directly inspires the design of EigenPro methods, which addressed the limitations of shallow learning caused by fast decaying eigenvalues.
%Third, 

==> expr/ob_eigenspectrum.tex <==
{\bf The Eigenspectrum of the Kernel Matrix.}
For each dataset, the eigenspectrum of the corresponding kernel matrix directly determines the impact of EigenPro on convergence. Thus we calculate a kernel matrix for each dataset by 4000 subsamples from it. Figure \ref{fig:es} presents the normalized eigenspectrums ($\lambda_i / \lambda_1$) of these kernel matrices. Eigenvalues in all curves drop sharply at the beginning, then become flatter in the middle. The concentration of the kernel spectrum on their top eigenspace makes EigenPro highly effective.
\begin{figure}[ht!]
    \centering
    
    \begin{subfigure}[t]{0.5\linewidth}
      \centering
       \includegraphics[width=\linewidth, scale=1.0]{expr/es_compare.png}
        \caption{\small Different data sets with subsample size $N = 4000$}
       \label{fig:es}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\linewidth}
      \centering
      \includegraphics[width=\linewidth,scale=1.0]{expr/es_compare_hint_m.png}
      \caption{\small Same data set, subsets of different sizes ($N$) }
      \label{fig:es-hint-m}
    \end{subfigure}%
    \caption{Eigenspectrum of the kernel matrices}
    % \label{fig:eigen}
\end{figure}


% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=\linewidth, scale=0.7]{es_compare.png}
%   \caption{Eigenspectrum of the Kernel Matrices}
%   \label{fig:es}
% \end{figure}

When EigenPro works on the top-$k$ eigen-directions, the multiplier of the step size is (the square root of) the ratio $\lambda_1 / \lambda_{k+1}$. To directly see the connection of $k$ and such multiplier, Table \ref{tbl:es-ratio} lists the eigenvalue ratio corresponding to different $k$. For example, with $k=160$, R-EigenPro can increase the step size of GD by 1063X for training HINT-M in theory.

\begin{table}[!htpb]
\centering
\caption{Eigenvalue ratio of kernel matrices}
\label{tbl:es-ratio}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Ratio & CIFAR & MNIST & SVHN & TIMIT & HINT-S \\ \hline
$\lambda_1 / \lambda_{41}$ & 62 & 66 & 36 & 52 & 117 \\ \hline
$\lambda_1 / \lambda_{81}$ & 113 & 124 & 65 & 103 & 186 \\ \hline
$\lambda_1 / \lambda_{161}$ & 196 & 242 & 116 & 202 & 311 \\ \hline
$\lambda_1 / \lambda_{321}$ & 321 & 443 & 201 & 310 & 674 \\ \hline
\end{tabular}
}%
\end{table}
The impact of EigenPro methods hinges on the approximation of the top eigensystem. Section \ref{sec:linear} claims that the top eigensystem of the kernel matrix can be restored with only a small subsample from the data. To verify this claim, Figure \ref{fig:es-hint-m} compares the eigenspectrums of the kernel matrices calculated from subsamples of HINT-M. The tightly overlapped region at the beginning of the curves supports the claim on efficiently restoring the top eigensystem.

==> expr/ob_macro.tex <==
\input{expr/macro_res.tex}

{\bf Convergence acceleration by EigenPro.}	
With an affordable time budget and small dataset, the computational reach of kernel methods often contains the optimal solution, such as the primal methods in Table~\ref{tbl:cmp-exact}. Our approach (P-EigenPro), in this case, is able to save $82\%$-$92\%$ epochs for reaching the optimal. Such saving persists even with random features (RF, R-EigenPro) where we converge to the optimal plus a bias introduced by the random feature sampling~\cite{rahimi2007random,dai2014scalable}.

When the resource/time budget is limited and the dataset is large,
the optimal solution is often out of the computational reach of kernel methods, such as the methods in Table~\ref{tbl:err-epoch}. Thus it is critical to expand the computational reach to contain a larger projection of the optimal with limited overhead. In this case, our approach (P-EigenPro and R-EigenPro) substantially decrease the error rate at the cost of up to $26\%$ more running time. Note that for complete MNIST-8M and HINT-M, the GPU memory can no longer hold the entire dataset as kernel centers, which disables the primal kernel methods. While the random methods do not suffer from such constraints. Moreover, using only $2\times 10^5$ random features, they well outperform the primal methods using $1 \times 10^6$ centers by training with more data.

==> expr/ob_overhead.tex <==
{\bf Overhead of EigenPro iteration.}
\label{sec:overhead}
\begin{wrapfigure}{r}{0.5\linewidth}
  \centering
  \includegraphics[width=1.1\linewidth, scale=1.4]{expr/overhead_primal.png}
%  \caption{Overhead per iter. }
 % \label{fig:overhead}
\end{wrapfigure}
Applying EigenPro preconditioner introduces computation and memory overhead. For standard SGD  using $D$ kernel centers (or random Fourier features) and mini-batch of size $m$, the computational cost per iteration is $O(m D)$. In comparison   for the EigenPro iteration using top-$k$ eigen-directions. computational cost becomes $O(mD+kD)$. The EigenPro method also need extra $k\cdot D$  memory to store the top-$k$ eigenvectors.
%\begin{figure}[!ht]

%\end{figure}
In practice, the computational overhead over the standard SGD  ranged between $10\%$ and $50\%$, not exceeding $30\%$ for 
$k \le 320$ used in our experiments on real data.
%in most cases.
See the figure  for details.
% compares the running time of SGD method with and without EigenPro over the same amount of epochs. The result indicates that (1) when $k$ is small ($\leq 320$), the overhead is a constant multiple of standard SGD running time, even when using half million points as kernel centers. (2) In our experiments, EigenPro with $k = 160$ introduces less than 20\% computational overhead per iteration, and EigenPro with $k = 320$ less than 30\% overhead.

==> expr/tbl_hint_gd.tex <==
\begin{table}[!ht]
\centering
\caption{Gradient descent (Pegasos) on HINT-M subset (10000 data points)}
\label{tbl:hint-gd}
\begin{adjustbox}{center}
\resizebox{15cm}{!}{
\begin{tabular}{|c|c||c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c||}{\multirow{2}{*}{Metric}} & \multicolumn{9}{c|}{Number of iterations} \\ \cline{3-11} 
\multicolumn{2}{|c||}{} & 1 & 5 & 20 & 80 & 320 & 1280 & 5120 & 10240 & 20480 \\ \hline
\multirow{2}{*}{L2 loss} & train & 8.25e-2 & 7.22e-2 & 5.72e-2 & 4.58e-2 & 3.75e-2 & 3.08e-2 & 2.30e-2 & 1.83e-2 & 1.32e-2 \\ \cline{2-11} 
 & test & 7.98e-2 & 7.02e-2 & 5.35e-2 & 4.24e-2 & 3.67e-2 & 3.34e-2 & 3.16e-2 & \textbf{3.14e-2} & 3.18e-2 \\ \hline
\hline
\multicolumn{2}{|c||}{$\left \| \alpha \right \|_2$} & 5.18e-2 & 1.73e-1 & 5.81e-1 & 1.89 & 6.44 & 22.7 & 79.7 & 1.46e2 & 2.62e2 \\ \hline
\end{tabular}
} \end{adjustbox}
\end{table}

==> linear/alg.tex <==
\begin{table*}[ht]
\begin{subalgorithm}{.5\textwidth}
%% EigenPro
\captionsetup{font=normalsize,singlelinecheck=off}
\caption{{\bf Algorithm:} $\mathrm{EigenPro}(X, \by, k, m, \eta$\\
$, \tau, M)$}\label{alg:linear-ep}
\begin{minipage}{.95\linewidth}
\begin{algorithmic}[1]
  \INPUT
	training data $(X, \by)$,
	number of eigen-directions $k$,
	mini-batch size $m$,
    step size $\eta$,
	damping factor $\tau$,
    subsample size $M$
  \OUTPUT
	weight of the linear model $\balpha$
  	\STATE $[E, \Lambda, \hat{\lambda}_{k+1}] = \mathrm{RSVD}(X, k+1, M)$
    \STATE $P \defeq I - E (I - \tau \hat{\lambda}_{k+1} \Lambda^{-1}) E^T$
    \STATE Initialize $\balpha \leftarrow 0$
  	\WHILE{stopping criteria is False}
    	\STATE $(X_m, \by_m) \leftarrow$ $m$ rows sampled from $(X, \by)$
        without replacement
        \STATE $\bg \leftarrow \frac{1}{m}(X_m^T (X_m \balpha) - X_m^T \by_m)$
%       \STATE $\bg \leftarrow \frac{1}{m}(\frac{1}{d}X_m^T (X_m \balpha) - \frac{1}{\sqrt{d}} X_m^T \by_m)$
  		\STATE $\balpha \leftarrow \balpha - \eta P \bg$
    \ENDWHILE
    
\end{algorithmic}
\end{minipage}
\end{subalgorithm}%

%% RSVD
\begin{subalgorithm}{.5\textwidth}
\captionsetup{font=normalsize,singlelinecheck=off}
\caption{{\bf Algorithm:} $\mathrm{RSVD}(X, k, M)$, adapted from \cite{halko2011finding}}\label{alg:rsvd}
\begin{minipage}{0.95\linewidth}
\begin{algorithmic}[1]
  \INPUT
    $n \times d$ matrix $X$,
    number of eigen-directions $k$,
    subsample size $M$
  \OUTPUT
  	$(\be_1(H_M),\ldots,\be_k(H_M))$,
    $\mathrm{diag}(\lambda_1(H_M), \ldots, \lambda_k(H_M)), \lambda_{k+1}(H_M)$
    %where $H_M$ is subsample covariance
  %%
    \STATE $X_M \leftarrow$ $M$ rows sampled from $X$ without replacement
    \STATE
    $[\lambda_1(X_M), \ldots, \lambda_{k+1}(X_M)]$, \\
    $[\bv_1(X_M),\ldots,\bv_{k}(X_M)]$ \\
    $\leftarrow rsvd(X_M, k+1)$,
    non-Hermitian version of Algorithm 5.6 in \cite{halko2011finding} ($\bv_i(X) \defeq $ $i$-th right singular vector)
    \STATE $\be_i(H_M) \leftarrow \bv_i(X_M)$ for $i = 1, \ldots, k$ \\
    $\lambda_i(H_M) \leftarrow \sqrt{\frac{n}{M}} \lambda_i(X_M)$ for $i \leq k+1$
    \newline
\end{algorithmic}
\end{minipage}
\end{subalgorithm}
\captionsetup{labelformat=alglabel}
\caption{EigenPro iteration for linear regression}%
\label{alg:epro}%
\end{table*}

% \begin{table}[ht]
% \begin{subalgorithm}{.5\textwidth}
% %% EigenPro
% \begin{algorithmic}[1]
% \ALG $\mathrm{EigenPro}(X, \by, k, m, \eta, c_0)$
%   \INPUT
% 	training data $(X, \by)$,
% 	number of eigen-directions $k$, \\
% 	mini-batch size $m$,
%     step size $\eta$,
% 	damping factor $\tau$, \\
%     subsample size $l$
%   \OUTPUT
% 	weight of the linear model $\balpha$
%   	\STATE $[E, \Lambda, \lambda_{k+1}] = \mathrm{RSVD}(X, k+1, s_0 \cdot k)$
%     \STATE $P \defeq I - E (I - \tau \lambda_{k+1} \Lambda^{-1}) E^T$
%     \STATE Initialize $\balpha \leftarrow 0$
%   %	\Statex
%   	\WHILE{stopping criteria is False}
%     	\STATE $(X_m, \by_m) \leftarrow$ $m$ rows sampled from $(X, \by)$ \\
%         without replacement
%         \STATE $\bg \leftarrow \frac{1}{m}(\frac{1}{d}X_m^T (X_m \balpha) - \frac{1}{\sqrt{d}} X_m^T \by_m)$
%   		\STATE $\balpha \leftarrow \balpha - \eta P \bg$
%     \ENDWHILE
% \newline
% \ALG $\mathrm{RSVD}(X, k, l)$, from \cite{halko2011finding}
%   \INPUT
%     $n \times d$ matrix $X$,
%     $k$,
%     sample size $l$
%   \OUTPUT
%   	$(\be_1(H_l),\ldots,\be_k(H_l)),
%     \mathrm{diag}(\lambda_1(H_l), \ldots, \lambda_k(H_l)),$ \\
%     $\lambda_{k+1}(H_l)$ where $H_l$ is a subsample covariance
% \end{algorithmic}
% \end{subalgorithm}%
% \captionsetup{labelformat=alglabel}
% \caption{EigenPro for linear regression}%
% \label{alg:epro}%
% \end{table}

==> linear/rsvd.tex <==
\begin{wraptable}{r}{0.5\linewidth}
\vspace{-5mm}

\begin{subalgorithm}{\linewidth}
\begin{algorithmic}[1]
\ALG $\mathrm{RSVD}(X, k, M)$, adapted from \cite{halko2011finding}
  \INPUT
    $n \times d$ matrix $X$,
    number of eigen-directions $k$,
    subsample size $M$
  \OUTPUT
  	$(\be_1(H_M),\ldots,\be_k(H_M))$,
    $\mathrm{diag}(\lambda_1(H_M), \ldots, \lambda_k(H_M)), \lambda_{k+1}(H_M)$
    %where $H_M$ is subsample covariance
  %%
    \STATE $X_M \leftarrow$ $M$ rows sampled from $X$ without replacement
    \STATE
    $[\lambda_1(X_M), \ldots, \lambda_{k+1}(X_M)]$, \\
    $[\bv_1(X_M),\ldots,\bv_{k}(X_M)]$ \\
    $\leftarrow rsvd(X_M, k+1)$,
    non-Hermitian version of Algorithm 5.6 in \cite{halko2011finding} ($\bv_i(X) \defeq $ $i$-th right singular vector)
    \STATE $\be_i(H_M) \leftarrow \bv_i(X_M)$ for $i = 1, \ldots, k$ \\
    $\lambda_i(H_M) \leftarrow \sqrt{\frac{n}{M}} \lambda_i(X_M)$ for $i \leq k+1$
    \newline
\end{algorithmic}
\end{subalgorithm}
\captionsetup{labelformat=alglabel}
\caption{RSVD}%
\label{alg:rsvd}
\vspace{-10mm}
\end{wraptable}

Given data matrix $X$, Algorithm RSVD computes its approximate top eigensystem using corresponding subsample covariance matrix $H_M \defeq \frac{1}{M} X_M^T X_M$. 
The algorithm has time complexity $O(Md\log{k} + (M + d) k^2)$ according to \cite{halko2011finding}.

The selection of subsample size $M$ depends on the eigenvalue decay rate of the covariance. Specifically, we choose $M = 4800$, which is much smaller than the size of training sets in our experiments. Thus, when $k = 160$, RSVD only takes a few minuets computation to complete even that the data (or kernel matrix) dimension $d$ exceeds $10^6$.
\newtxtblock

==> misc/tbl_bound.tex <==
\begin{table}[!ht]
\centering
\caption{Cost and convergence bound of several first/second order methods}
\label{my-label}
\resizebox{17cm}{!}{
\begin{tabular}{|c|c|c|c|l|c|}
\hline
Method & \begin{tabular}[c]{@{}c@{}}Cost per\\ iteration\end{tabular} & \begin{tabular}[c]{@{}c@{}}Maintenance\\ Overhead\end{tabular} & \begin{tabular}[c]{@{}c@{}}Storage\\ Overhead\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Convergence Iteration (t)\\ s.t. $L(\alpha_t) - L(\alpha^*) \leq \epsilon$\\ or $\mathbb{E}[L(\alpha_t) - L(\alpha^*)] \leq \epsilon$\end{tabular}} & Note \\ \hline
GD & $O(nld)$ & - & - & \begin{tabular}[c]{@{}l@{}}$O(\kappa(H) \log{\frac{1}{\epsilon}})$~\cite{dennis1996numerical}\\ $O(\sqrt{\kappa(H)} \log{\frac{1}{\epsilon}})$~\cite{frostig2015regularizing}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$nld$ can easily exceed $10^9$\\ in large-scale shallow learning.\end{tabular} \\ \hline
SGD & $O(mld)$ & - & - &  & \begin{tabular}[c]{@{}c@{}}constant $\eta$, no $\lambda_d$, weight averaging~\cite{bach2013non};\\ decaying $\eta_t$, $\kappa(H)$~\cite{nemirovski2009robust};\\ constant $\eta$, complicated~\cite{murata1998statistical}.\end{tabular} \\ \hline
AdaGrad & $O(mld + ld)$ & \begin{tabular}[c]{@{}c@{}}$O(ld)$\\ per iteration\end{tabular} & $O(ld)$ & \cite{duchi2011adaptive} & Rescale the gradient coordinate-wisely. \\ \hline
L-BFGS & $O(nld + kld)$ & \begin{tabular}[c]{@{}c@{}}$O(kld)$\\ per iteration\end{tabular} & $O(ld)$ & $O(r \log{\frac{1}{\epsilon}})$ where $0 \leq r < 1$~\cite{liu1989limited} & \begin{tabular}[c]{@{}c@{}}Each iteration involves a two-loop recursion\\ that is difficult to be parallelized.\end{tabular} \\ \hline
sL-BFGS & $O(mld + kld)$ & \begin{tabular}[c]{@{}c@{}}$O(Mld)$\\ per $T_1$ iterations\end{tabular} & $O(kld)$ & $O(\frac{Q(\beta)}{\epsilon})$~\cite{byrd2016stochastic} & \begin{tabular}[c]{@{}c@{}}Typically has $M \geq 300, k = 5, T_1 = 20$.\\ Use the subsample covariance $H_M$.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Subsample\\ Newton\end{tabular} & $O(nld + kld)$ & \begin{tabular}[c]{@{}c@{}}$O(Mld)$\\ per iteration\end{tabular} & $O(kld)$ & \cite{erdogdu2015convergence} & Works with full gradient. \\ \hline
LiSSA & $O(nl + S_1 \kappa) d$ & - & $O(S_1 d)$ & $O(\log^2\frac{1}{\epsilon} \log\log\frac{1}{\epsilon})$~\cite{agarwal2016second} &  \\ \hline
\begin{tabular}[c]{@{}c@{}}EigenPro\\ iteration\end{tabular} & $O(mld + kld)$ & \begin{tabular}[c]{@{}c@{}}$Md\log{k}$ \\ $+ (M+d)k^2$\\ one time\end{tabular} & $O(kd)$ &  &  \\ \hline
\end{tabular}
}%
\end{table}

==> preliminary/fig_iter_eigen.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \vspace{-5mm}
  \centering
  \includegraphics[width=0.5\textwidth]{figs/nit_HINT-M_max_200_eps_4_l_4.png}
  %{figs/mnist_y_proj_e_lb_n_4.png}
  \caption{Iterations needed for converging to label vectors along each eigendirection (estimated by Eq.~\ref{eq:gd_number_iterations_i} with $\epsilon =  10^{-4}$, $10^4$ data points from HINT-M dataset)}
  \label{fig:proj-iter}
  \vspace{-5mm}
\end{wrapfigure}

==> shallow.tex <==
\section{EigenPro for  Scalable Kernel Methods}
\label{sec:shallow}
While EigenPro iteration can be applied to any linear regression problem, the maximum benefit is obtained when the feature space is very high-dimensional, particularly in conjunction with smooth kernels. 
We will briefly discuss two standard kernel-related feature maps as well as well some modifications needed to work directly in the RKHS (primal) setting. \newtxtblock

% EigenPro preconditioning method, which works for the linear setting in Section~\ref{sec:linear}, can be applied to a general shallow learning setting, and especially, several scalable kernel methods.

% Consider LLS (Eq.~\ref{eq:lls}) incorporated with feature map $\phi: \mathbb{R}^d \rightarrow \mathbb{R}^D$ that embeds a data point $x \in X$ into $\mathbb{R}^D$,
% \begin{equation} \label{eq:lls-phi}
% L_{\phi}(\balpha) \defeq \frac{1}{n} \sum_{i=1}^{n} {(
% %\frac{1}{\sqrt{D}} 
% \langle \balpha, \phi(x_i) \rangle - y_i)^2}
% \end{equation}
% It corresponds to regression
% $\balpha^* = \arg\min_{\balpha \in \mathbb{R}^D}{L_{\phi}(\balpha)}$.
% Such regression problem leads to a general shallow learning framework that could cooperate with powerful non-linear feature embeddings, e.g. reproducing kernel.

% Essentially, the regression problem with feature map $\phi(\cdot)$ is equivalent to LLS involving $n \times D$ data matrix $\Phi \defeq (\phi(x_1), \ldots, \phi(x_n))^T$. Therefore, we can apply the EigenPro preconditioned SGD to this shallow learning problem
% by performing algorithm $\aEP$ (Table~\ref{alg:linear-ep}) on the new data matrix, $\Phi$. Note that since $D$ could be much larger than $d$, data matrix $\Phi$ is never materialized as a whole. Instead, data points in $\Phi$ are materialized on the fly, e.g. mini-batch for SGD and subsample data matrix for algorithm $\aRSVD$ (Table~\ref{alg:rsvd}).
% Here we consider the following three feature maps based on RKHS kernel.

%%%%%%%%%%% 
% When the feature map is induced by a reproducing kernel, the above regression becomes kernel least squares regression (KLS).
% Two kernel methods, ``RBF network'' (RBF)~\cite{queback} and random Fourier features with $L^2$ loss (RFF)~\cite{rahimi2007random} are KLS with different feature maps.
% What's more, when $\phi$ is a kernel function, it maps $x$ to an RKHS space with infinite dimension. 
% Note that the special properties of RKHS~\cite{bishop2006pattern} make such generalization ($D \rightarrow \infty$) valid.

% The rest of this section will detail how EigenPro preconditioning works with several popular kernel methods: (1) for kernel methods involving finite dimensional feature map (e.g. RBF and RFF), we specify the feature map, $\phi(\cdot)$, so that algorithm $\mathrm{EigenPro}$ (Table~\ref{alg:linear-ep}) can be applied to $\Phi$ materialized on demand; (2) for kernel methods involving infinite dimensional feature map (e.g. to RKHS space), extra parametrization is required which leads to variant of algorithm $\aEP$ (Table~\ref{alg:primal-ep}).
\noindent {\bf Random Fourier features (RFF)~\cite{rahimi2007random}.}
The random Fourier feature map $\mathbb{R^N}\to \mathbb{R^d}$ is defined by
% to a shift invariant kernel $\rmk(\bx, \bx') = \rmk(\bx - \bx')$ for $\bx, \bx' \in \mathbb{R}^d$,
%\begin{equation} \label{eq:rff}
$$
\phi_{\mathrm{rff}}(\bx) \defeq \sqrt{2d^{-1}}(\cos(\bomega_1^T\bx + b_1), \ldots, \cos(\bomega_d^T\bx + b_d))^T
$$
%\end{equation}
Here $\bomega_1, \dots, \bomega_d$ are  sampled from the distribution $\frac{1}{2\pi} \int{\exp(-j \bomega^T \delta)\rmk(\delta)}{d\Delta}$ and $b_1, \ldots, b_d$ from uniform distribution on $[0, 2\pi]$.
It can be shown that the inner product in the feature space approximates  a Gaussian kernel $\rmk(\cdot, \cdot)$, i.e.,
%\begin{equation} \label{eq:rff-kernel}
$\lim_{D \rightarrow \infty}{\phi_{\mathrm{rff}}(\bx)^T \phi_{\mathrm{rff}}(\by)} = \rmk(\bx, \by)$.
%\end{equation}
\newtxtblock

\noindent {\bf Radial basis function network (RBF) features.}%~\cite{queback,camoriano2016nytro}.} 
This setting involves feature map related to kernel $\rmk(\cdot, \cdot)$, defined as
%\begin{equation} \label{eq:rbf}
$$
\phi_{\mathrm{rbf}}(\bx) \defeq
(\rmk(\bx, \bz_1), \dots, \rmk(\bx, \bz_d))^T
$$
%\end{equation}
where $\{ z_i \}_{i=1}^{d}$%, $z_i \in \mathbb{R}^d$
are network centers. Note there are various strategies for selecting centers, e.g., randomly sampling from $X$~\cite{camoriano2016nytro} or by computing K-means centers leading to different interpretations in terms of data-dependent kernels~\cite{queback}.
%%%%%%
\newtxtblock

\noindent {\bf EigenPro iteration in RKHS (primal).}
In this setting, a reproducing kernel $\rmk(\cdot, \cdot): \mathbb{R}^N \times \mathbb{R}^N \rightarrow \mathbb{R}$ implies a feature map from $X$ to an RKHS space $\mathcal{H}$ (typically) of infinite dimension. The feature map can be written as  $\phi:  x \mapsto k(x, \cdot), \mathbb{R}^N \to \mathcal{H}$.
%Given reproducing kernel $\rmk(\cdot, \cdot): \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$, consider feature map $\rmk(\cdot, \cdot): \mathbb{R}^d \rightarrow \mathcal{H}$ where $\mathcal{H}$ is the corresponding RKHS space~\cite{bishop2006pattern}. Then define the empirical loss on $\mathcal{H}$,
This feature map leads to the (shallow) learning problem
$$
f^*=\arg\min_{f \in \mathcal{H}} \frac{1}{n} \sum_{i=1}^{n} {( \langle f, \rmk(\bx_i, \cdot) \rangle_{\mathcal{H}} - y_i)^2}
$$
Using properties of RKHS, EigenPro iteration in $\HH$ becomes $f \leftarrow f - \eta \rmP (\rmH(f)- \rmb)$
where $\rmb \defeq \frac{2}{n} \sum_{i=1}^n {y_i k(\bx_i, \cdot)}$ and covariance operator
$\rmH \defeq \frac{2}{n} \sum_{i=1}^n{\rmk(\bx_i, \cdot) \otimes \rmk(\bx_i, \cdot)}$.
The top eigensystem of $\rmH$ forms the preconditioner
$\rmP \defeq \rmI - \sum_{i=1}^{k}{(1 -\tau\frac{\lambda_{k+1}(\rmH)}{\lambda_i(\rmH)}) \rme_i(\rmH) \otimes \rme_i(\rmH)}$.
\newtxtblock
\input{shallow/alg}
Notice that by the Representer theorem~\cite{aronszajn1950theory}, $f^*$ admits a representation of the form $\sum_{i=1}^{n}{\alpha_i \rmk(\bx_i, \cdot)}$.
Parameterizing the above iteration accordingly and applying some linear algebra lead to the following iteration in a finite-dimensional vector space,
$$
\balpha \leftarrow \balpha - \eta P (K \balpha - \by)
$$ 
where $K \defeq [\rmk(\bx_i, \bx_j)]_{i,j = 1, \ldots, n}$ is the kernel matrix and EigenPro preconditioner $P$ is defined using the top eigensystem of $K$ (assume $K\be_i = \lambda_i \be_i$),
$$
P \defeq I - \sum_{i=1}^k
{\frac{1}{\lambda_i}
(1 - \tau \frac{\lambda_{k+1}}{\lambda_i}) \be_i \be_i^T}
$$

This preconditioner differs from that for the linear case (Eq.~\ref{eq:epro-pc}) due to the parametrization in RKHS space. Table~\ref{alg:primal-ep} details the SGD version of this iteration.

% To perform EigenPro iteration on $\alpha$ in SGD setting, we first transform mini-batch $(X_m, \by_m)$ to batch $(K_m \leftarrow k(X_m, X), \by_m)$. Let $\balpha_m \defeq$ portion of $\balpha$ corresponding to $K_m$ and calculate $m$-dimensional gradient vector $\bg_m \leftarrow \frac{1}{m}(\frac{1}{\sqrt{n}} K_m \balpha - \by_m)$. One EigenPro iteration then update $\alpha$ in two steps: $\balpha_m \leftarrow \balpha_m - \eta \bg_m$, $\balpha \leftarrow \balpha + \eta D\bg_m$.


% Similar to the linear EigenPro iteration, the RKHS version can increase the step size by a factor of $\sqrt{\frac{\lambda_1}{\lambda_{k+1}}}$ over that of the standard SGD. (we skip the analysis due to space limitation) More details on applying this iteration can be found in Table~\ref{alg:primal-ep}. 

% $f^*$ can be obtained by solving the functional system, $\rmH(f) - \rmb = 0$,
% with $\rmb \defeq \frac{2}{n} \sum_{i=1}^n{y_i \rmk(\bx_i,\cdot)}$ and 
% $\rmH(f) \defeq \frac{2}{n} \sum_{i=1}^{n}{\left\langle \rmk(\bx_i, \cdot), f \right\rangle_\mathcal{H} \rmk(\bx_i, \cdot)}$.
% Assume that $\rmH = \sum_{i=1}^{n}{\lambda_i \rme_i(\cdot) \otimes \rme_i(\cdot)}$
% with $\lambda_1 \geq \ldots \geq \lambda_n$ is its eigendecomposition.
% Then the EigenPro iteration corresponding to the functional system has the form,
% $f \leftarrow f - \eta \rmP (\rmH(f)- \rmb)$
% with EigenPro preconditioner, 
% $\rmP \defeq \rmI - \sum_{i=1}^{k}{(1 - \frac{\lambda_{k+1}}{\lambda_i}) \rme_i(\cdot) \otimes \rme_i(\cdot)}$.

% Notice that both $f^*(\cdot)$ (by Representer theorem~\cite{aronszajn1950theory}) and $\rme_i(\cdot)$ (by definition) admit a representation in terms of function set $\{ k(\bx_i, \cdot) \}_{i=1}^n$. Such representation allows us to parametrize the functional EigenPro iteration into an iteration over $n$-dimensional vector space. In addition, we have
% $(\rmH\rme_i)(\cdot)
% = \frac{\lambda_i(K)}{n} \rme_i(\cdot)
% = \frac{1}{n}  \sum_{j=1}^{n} {\rme_i(\bx_j) \rmk(\bx_j, \cdot)}$
% where $K \defeq [\rmk(\bx_i, \bx_j)]_{i,j = 1, \ldots, n}$ is the kernel matrix. This suggests us to restore the top eigensystem of $\rmH$ by that of $K$.

% Finally, the parametrized EigenPro iteration is presented in Table~\ref{alg:primal-ep}. Its impact on step size and convergence is similar to that of the linear case (a similar analysis is skipped due to space limitation). When using the top-$k$ eigensystem, the EigenPro iteration can increase the step size by a factor of $\sqrt{\frac{\lambda_1}{\lambda_{k+1}}}$ over that of the standard iteration.

%Its impact on learning rate and convergence for both GD and SGD follows an analysis similar to that for the linear case in Section~\ref{sec:step}.

% The corresponding kernel methods then aim to solve the following regression problem in an RKHS space,
% \begin{equation} \label{eq:lls-primal}
% f^*=\arg\min_{f \in \mathcal{H}} \frac{1}{2n} \sum_{i=1}^{n} {( \langle f, \rmk(\bx_i, \cdot) \rangle_{\mathcal{H}} - y_i)^2}
% \end{equation}

%Note that a regularization term, e.g. $\norm{f}_\mathcal{H}$, is needed in the above regression to avoid overfitting. However, in gradient-based methods  early stopping has similar regularization effects and is often preferable from the computational point of view~\cite{camoriano2016nytro}.

% By properties of RKHS, 
% $f^*$ can be obtained by solving the functional system, $\rmH(f) - \rmb = 0$,
% with $\rmb = \sum_{i=1}^n{y_i \rmk(\bx_i,\cdot)}$ and $\rmH: \mathcal{H} \rightarrow \mathcal{H}$, the covariance operator, defined as
% \begin{equation} \label{eq:rkhs-cov}
% \rmH(f) \defeq \frac{1}{n} \sum_{i=1}^{n}{\left\langle \rmk(\bx_i, \cdot), f \right\rangle_\mathcal{H} \rmk(\bx_i, \cdot)}
% \end{equation}
% Similar to the linear case in Section~\ref{sec:linear}, the solution of the system can be approximated by preconditioned gradient descent,
% \begin{equation}\label{eq:gd-primal}
% f \leftarrow f - \eta \rmP (\rmH(f)- \rmb)
% \end{equation}
% with invertible operator $\rmP: \mathcal{H} \rightarrow \mathcal{H}$ as the preconditioner. Assume $\rmH$ has eigendecomposition

% $\rmH = \sum_{i=1}^{n}{\lambda_i \rme_i(\cdot) \otimes \rme_i(\cdot)}$
% with $\lambda_1 \geq \ldots \geq \lambda_n$. Then we can construct the EigenPro preconditioner for iteration Eq.~\ref{eq:gd-primal}, defined as
% \begin{equation} \label{eq:rkhs-epro}
% \rmP \defeq \rmI - \sum_{i=1}^{k}{(1 - \frac{\lambda_{k+1}}{\lambda_i}) \rme_i(\cdot) \otimes \rme_i(\cdot)}
% \end{equation}
% whose second term is a rank-$k$ operator. 

% To apply iteration Eq.~\ref{eq:gd-primal} in practice, we need a representation of $f$ in a space with finite dimension. 
% Notice that $\rmP (\rmH(f) - \rmb)$ is a linear combination of functions within $\{ \rmk(\bx_i, \cdot) \}_{i=1}^n$. In fact, according to the Representer theorem~\cite{aronszajn1950theory}, $f^*$ must have the form,
%regularized $L_{\rmk(\cdot, \cdot)}(f)$ the minimizer $f^*$ has the form
% \begin{equation} \label{eq:rep-primal}
% f^*(\cdot) \defeq \sum_{i=1}^{n}{\alpha_i \rmk(\bx_i, \cdot)}
% \end{equation}
% $f^*(\cdot) \defeq \sum_{i=1}^{n}{\alpha_i \rmk(\bx_i, \cdot)}$
% where $\balpha = (\alpha_1, \ldots, \alpha_n)^T$ is the vector of coefficients in the representation of $f$ in terms of  $\{ \rmk(\bx_i, \cdot) \}_{i=1}^n$.

% Note that $\rme_i(\cdot)$ also admits a representation in terms of function set $\{ k(\bx_i, \cdot) \}_{i=1}^n$.
% Thus,
%\begin{equation} \label{eq:rkhs-cov-eigen-prop}
% $$
% (\rmH\rme_i)(\cdot)
% = \frac{\lambda_i(K)}{n} \rme_i(\cdot)
% = \frac{1}{n}  \sum_{j=1}^{n} {\rme_i(\bx_j) \rmk(\bx_j, \cdot)}
% $$
%\end{equation}
%where $K \defeq [\rmk(\bx_i, \bx_j)]_{i,j = 1, \ldots, n}$ is the kernel matrix.
%and $(\rme_i(\bx_1), \ldots, \rme_i(\bx_n))^T$ is its i-th eigenvector. 
%Such connection implies that it is feasible to restore the top-eigensystem of $\rmH$ by that of $K$.

% Finally, we can rewrite the iteration Eq.~\ref{eq:gd-primal} on function $f$ as iteration on vector $\balpha$.
% Let $[E, \Lambda, \lambda_{k+1}] \leftarrow \mathrm{RSVD}(K, k+1, l)$. Then replacing $\{ \rme_i(\cdot) \}_{i=1}^n$, $\rmb(\cdot)$, and $f(\cdot)$ by their representations under $\{ \rmk(\bx_i, \cdot) \}_{i=1}^n$, iteration Eq.~\ref{eq:gd-primal} becomes
% \begin{equation}\label{eq:gd-primal-rep}
% \balpha \leftarrow \balpha - \eta P (K \balpha - \by)
% \end{equation}
% where $P = I - E(n\Lambda^{-1})(I - \lambda_{k+1} \Lambda^{-1})E^T$ is the preconditioner for the new iteration. The preconditioner differs from that of the linear case in Table~\ref{alg:linear-ep}. Especially, it has an extra $n\Lambda^{-1}$ term due to the adoption of RKHS inner product in Eq.~\ref{eq:lls-primal} instead of the $L^2$ inner product in Eq.~\ref{eq:lls-phi}.
% What's more, the SGD version of this iteration needs to update $\balpha$ in two steps instead of one step as in the linear case. See algorithm in Table~\ref{alg:primal-ep} for details. 

